Everything is Relative: Understanding Fairness with Optimal Transport

To study discrimination in automated decision-making systems, scholars have proposed several definitions of fairness, each expressing a different fair ideal. These definitions require practitioners to make complex decisions regarding which notion to employ and are often difficult to use in practice since they make a binary judgement a system is fair or unfair instead of explaining the structure of the detected unfairness. We present an optimal transport-based approach to fairness that offers an interpretable and quantifiable exploration of bias and its structure by comparing a pair of outcomes to one another. In this work, we use the optimal transport map to examine individual, subgroup, and group fairness. Our framework is able to recover well known examples of algorithmic discrimination, detect unfairness when other metrics fail, and explore recourse opportunities.

==> old files/compute.tex <==
\subsection{Computational Aspects}
In this section we present an algorithm for computing comparative fairness on the individual, subgroup, and group level as well as some assumptions we made to make the problem tractable. 

%We assume that the exact measure corresponding to $\X$ is unknown, and so we approximate this distribution by assuming the existence of a random sample $X = \{(x_{i}\}_{i=1}^{n} \sim \mathcal{X}$. Suppose we can split the data into two groups $A$ and $B$ and apply the policies $\Policy_{0}$ and $\Policy_{1}$ to respectively.  We approximate $\mu_{\Policy_{0}}$ by observing the set of outcomes generated by applying $\Policy_{1}$ on all $a \in A$, assuming each $\Policy_{1}(a)$ is also observed with uniform probability. The distribution $\mu_{\Policy_{1}}$ to be the distribution is approximated similarly.  Finally, approximate the wasserstein distance $ \Wass_{p}(\mu_{\Policy_{1}}^{A}, \mu_{\Policy_{2}}^{B})$ between these approximated distributions is computed. 



We can use the Wasserstein distance $\Wass_{p}(\mu_{\Policy_{1}}, \mu_{\Policy_{2}})$ to measure the difference between the policies and recover the optimal coupling $\optcpl$. Since $\mu_{\Policy_{1}}$ and $\mu_{\Policy_{2}}$ are uniformly distributed over possible outcomes, the cost function $c$ used in the wasserstein computation is the is the $L^1$ distance between outcome probabilities.  When we are dealing with samples of finite sample size, the cost matrix is given by:
\begin{equation}
    C_{ij} = \norm{ \Policy_{1}(a_{i}) -  \Policy_{2}(b_{i}) }
\end{equation}
Whereas the optimal coupling is the solution to (5).  \kweku{should we write down the linear program?} 

Using the optimal coupling, it is easy to compute our individual and subgroup fairness metrics.  

%  

% \rebecca{Insert toy example here}

% \subsection{Measuring Group and Individual Fairness}

% To understand whether or not policies are fair, we need to measure their impact on both the individual and group levels. In the context of optimal transport, we would like to study which individuals are mapped to one another between classes. For individual $x^0_i,$ define $\gamma(x^0_i) $ to be the group of individuals in the other class that $x^0_i$ is mapped to:
% \begin{equation}
%     \gamma(x^0_i)  = \{ j : \ \Gamma_{ij} > 0 \}.
% \end{equation}

% Suppose we are able to quantify how different individuals are with some distance $d$. For example, $d$ could measure \rebecca{use whatever running example from the toy problem}. Note that in the worst case scenario, an individual will have all of their mass mapped to the individual in the opposite class who is farthest from them. Thus, to measure how unfair the outcome is for individual $x^0_i$ with respect to a distance $d$, we can take a weighted average over the distances between individual $x^0_i$ and those they are mapped to and normalize it by their own worst-case-scenario:
% \begin{equation}
%     u_d(x^0_i) = \frac{n \sum_{j=1}^m \Gamma_{ij} d(x^0_i, x^1_j)}{\max_{j = 1:m} d(x^0_i, d^1_j)}.
% \end{equation}
% To measure unfairness for the whole group, we simply need to average the individual scores:
% \begin{equation}
%     U_d(X^0) = \frac{1}{n} \sum_{i=1}^n u_d(x^0_i).
% \end{equation}

% While the above framework is presented for comparing the two groups $X^0$ and $X^1,$ it can easily be modified to compute the differences between subgroups. 



The success the above framework relies on the existence of a metric $d: \mathcal{X} \rightarrow \mathcal{X}$ which suitably can compute differences between individuals.  Although $(X,d)$ is a metric space and most euclidean norms suffice, we leave the choice in distance metric as a hyper-parameter in our problem formulation.  Across settings, vectorized representations of individuals may suffer from differences that necessitate the use of a some custom or non-euclidean metric.  In our experiments we use a normalized euclidean metric:
\begin{equation}
 u_{X}(a) =  \frac{\sum_{\substack{b \in \X, \\ b \in \pi(a,\optcpl)}}d(a,b)\optcpl(a,b)}{\max_{b \in \X} d(a, b)}
\end{equation}

that looks to normalize each individual's distances by the largest possible 


==> old files/context.tex <==
\section{Background}
Allow $\X \subseteq \Reals{d}$ to be some set of features and $\Y = \binaryset$ to be some binary set of possible outcomes for some decision. For now, we assume that $\A = \binaryset$ is the variable describing the protected group membership of an individual. In the binary case, a classifier is represented by a function $h: \X \rightarrow \binaryset$ which outputs a classification decision $h(\x)$ for a given individual $\x \in \X$.  We assume there exists a distribution $\mathcal{D}$ over the set $\mathcal{Z} = \X \times \A \times \Y$, which takes on values  $(x,a,y)\sim\mathcal{D}$. 

% \begin{definition}[Demographic Parity]
% A classifier is fair under Demographic Parity if the classifier's predictions are independent from sensitive attribute membership. 
% \begin{align}
%     \Expect{\mathcal{D}}[h(X)|A=1] = \Expect{(\mathcal{D}}[h(X)|A=0]  
% \end{align}
% \end{definition}

% Note that this is simply a statement of equality and does not reveal the quantity of observed deviation from a fair ideal, should such a deviation exist and the condition remain unsatisfied.  Requiring Demographic Parity allows the system planner to observe if something is fair or not, but this simple binarized check lacks nuance, which may be crucial to the problem domain.  In some cases, bias is the result of a protected attribute attribute being correlated with an individual's labeling.  In this case, by ignoring the underlying structure of the bias, demographic parity can decrease overall classifier if \kweku{cite fair svm and too relaxed}:
% \begin{align*}
%     Pr[Y=y|A=1] \neq Pr[Y=y|A=0] \quad \forall (x,a,y) \in \mathcal{Z}
% \end{align*}
% To address the strictness of independence assumptions made by demographic parity, others have attempted a relaxed version of demographic parity called Difference of Demographic Parity (DDP):
% \begin{align*}
%     DDP(f) \coloneqq \Expect{\mathcal{D}}[h(X)|A=1] - \Expect{\mathcal{D}}[h(X)|A=0] 
% \end{align*}

% Although the $DDP(h)$ can help describe the extent to which demographic parity is satisfied, it can hardly suffice as a fairness measurement as it provides little in the way of explaining the structure of the observed bias. 

% Other statistical fairness notions exist to address some of the shortcomings of demographic parity.  For example we will also consider equal opportunity, which enforces fairness as an equalization of true positive rates of a classifier.  

% \begin{definition}[Equal Opportunity]
% \begin{align*}
% \Expect{\mathcal{D}}[h(X)|Y=1, A=1] = \Expect{\mathcal{D}}[h(X)|Y=1, A=0]  
% \end{align*}
% \end{definition}
% \kweku{say some words about how equal}



% Allow $\simp$ to be the two dimensional probability simplex. We view a classifier as a deterministic mapping $f:\X \rightarrow \simp$ from the set of features to the set of possible distributions over outcomes, each being a point within the two dimensional simplex.  \kweku{this assumption needs to be justified, the simplex thing}






\kweku{Talk here about fairness being about distributions not specific decisions}

\kweku{Does this mapping always exist on a dataset, on a classifier? Does it need to be smooth/continuous? How is that defined?}



==> old files/ot.tex <==
\section{Optimal Transport}
Optimal transport seeks to find the most cost-effective way to transform one probability distribution into another \cite{peyre2019computational}.  The Kantorovich formulation allows the transport map to split masses between domains, meaning that the map does not need to be a bijection. Formally, given two measures $\mu$ and $\nu$ defined on the measure space $\X$, respectively, the optimal transport problem seeks to find the optimal coupling $\pi$ that attains
\begin{equation}
    \min_{\pi \in \Pi(\mu, \nu)} \int_{\X \times \X} c(x, y)  d \pi(x, y),
    \label{ot}
\end{equation}
where $c(x, y)$ is a cost function and $\Pi(\mu, \nu) $ is the set of couplings of $\mu$ and $\nu$ given by:
\kweku{Make couplings behave}
% \begin{align}
%     \Pi(\mu, \nu) = \{ \pi \in P(\mathcal{X} \times \mathcal{Y}) : \pi(A \times \mathcal{Y}) = \mu(A) \text{ for }  A \subset \mathcal{X}, \ \pi(\mathcal{X} \times B) = \nu(B) \text{ for } B \subset \mathcal{Y} \}. 
% \end{align}
. The $p$th Wasserstein distance is a special case of this optimal transport problem when the cost function is given by $c(x,y) = d(x,y)^p$, where $d:\X \rightarrow \X$ is some distance function. 
\begin{equation}
      W_{p}(\mu, \nu) \equiv \left(\inf_{\pi\in \Pi(\mu,\nu)} \int_{\mathcal{X} \times \mathcal{X}} d(x^0, x^1)^{p} d\pi(x^0,x^1)\right)^{\frac{1}{p}}.
      \label{Wasserstein}
\end{equation}

In the discrete setting, given data $X^0 = (x^0_1, x^0_2, \dots, x^0_{n})$ from $\mathcal{X}^0$ and $X^1 = (x^1_1, x^1_2, \dots, x^1_{m})$ from $\mathcal{X}^1$, the the marginal distributions can be expressed as 
\begin{equation*}
    p = \sum_{i=1}^{n} p_i \delta_{x^0_i} \text{ and } q = \sum_{j=1}^{m} q_j \delta_{x^1_j},
\end{equation*}
where $\delta_{x}$ is the Dirac measure. Similarly, the cost can be described as a matrix $C \in \mathbb{R}^{n \times m} $, where $C_{ij} = c(x^0_i, x^1_j)$, and the set of admissible couplings are the matrices 
\begin{equation}
    \Pi(p,q) = \{ \Gamma \in \mathbb{R}_+^{n \times m} : \Gamma \mathds{1}_{m} = p, \ \Gamma^T \mathds{1}_{n} = q \}. 
\end{equation}
Then, the discrete optimal transport problem is
\begin{equation}
    \min_{\Gamma \in \Pi(p,q)} \langle \Gamma, C \rangle.
    \label{discreteOT}
\end{equation}



% We are interested in quantifying the differences in outcomes for individuals from different protected classes. Suppose we can split the data into two groups $X^0$ and $X^1$ and apply the policies $\Policy_0$ and $\Policy_1$ to their respective class. Allow $\mu(\Policy_{0}(X^0))$ denoted $\mu_{0}(\Policy_{0})$ to be the distribution generated by observing policy $\Policy_{0}(X^0)$ on group $X_0$, and define $\mu_1(\Policy_1)$ similarly. 

% We can use the Wasserstein distance $W_p(p,q)$ to measure the difference between the policies and recover the coupling $\Gamma$. We set $p$ and $q$ to be the uniform distributions over the individuals, and the cost matrix $C$ is the $L^1$ distance between outcome probabilities:
% \begin{equation}
%     C_{ij} = \norm{\mu_0(\Policy_0(x^0_i)) -  \mu_1(\Policy_1(x^1_j))}_1 .
% \end{equation}
% This Wasserstein distance measures the most cost-effective way to split the mass of the outcomes for group $X^0$ onto the outcomes for group $X^1$, effectively transforming one distribution into the other. By comparing outcome probabilities, each entry $\Gamma_{ij}$ in the coupling matrix tells us how similar individual $x^0_i$ is to individual $x^1_j$ as measured by the policies.

% \rebecca{Insert toy example here}

% \subsection{Measuring Group and Individual Fairness}

% To understand whether or not policies are fair, we need to measure their impact on both the individual and group levels. In the context of optimal transport, we would like to study which individuals are mapped to one another between classes. For individual $x^0_i,$ define $\gamma(x^0_i) $ to be the group of individuals in the other class that $x^0_i$ is mapped to:
% \begin{equation}
%     \gamma(x^0_i)  = \{ j : \ \Gamma_{ij} > 0 \}.
% \end{equation}

% Suppose we are able to quantify how different individuals are with some distance $d$. For example, $d$ could measure \rebecca{use whatever running example from the toy problem}. Note that in the worst case scenario, an individual will have all of their mass mapped to the individual in the opposite class who is farthest from them. Thus, to measure how unfair the outcome is for individual $x^0_i$ with respect to a distance $d$, we can take a weighted average over the distances between individual $x^0_i$ and those they are mapped to and normalize it by the worst-case-scenario:
% \begin{equation}
%     u_d(x^0_i) = \frac{n \sum_{j=1}^m \Gamma_{ij} d(x^0_i, x^1_j)}{\max_{j = 1:m} d(x^0_i, d^1_j)}.
% \end{equation}
% To measure unfairness for the whole group, we simply need to average the individual scores:
% \begin{equation}
%     U_d(X^0) = \frac{1}{n} \sum_{i=1}^n u_d(x^0_i).
% \end{equation}

% While the above framework is presented for comparing the two groups $X^0$ and $X^1,$ it can easily be modified to compute the differences between subgroups. 


==> old files/toy.tex <==
\section{Toy Example}
We motivate the usage of the Wasserstein Distance for fairness evaluation with the following example. The fictitious and prestigious Blue College is looking to audit their admissions data for bias. In general Blue's applicants come from two secondary schools: expensive private School A, and the less-expensive public School B.  Blue College would like to check that their admissions policy is not biased with respect to an applicant's school. We assume that the college can estimate the likelihood $P(Y=1|X=x)$ for a given student with GPA $x \in X$ to be admitted into the college based on previous data. Looking at their admissions data, Blue College observes the following admission rule:
\begin{enumerate}
    \item For \textit{all} students in School A, the probability of being accepted to Blue College is $P(Y=1|X=x) = P(Y=1) = 0.15$. 
    \item For students in School B, the probability of being accepted is $P(Y=1|X=x) = 1$ for the students with GPAs in the top 15\% of GPAs in their class, and $P(Y=1|X=x) = 0$  for the bottom 85\%.
\end{enumerate}

Suppose the school wishes to be fair according to the disparate impact criteria.  
\theoremstyle{definition}
\begin{definition}[Disparate Impact (80\% Rule)]
A model is said to admit disparate impact if:
\begin{align}
    \frac{P(Y=1|School=B)}{P(Y=1|School=A)} \leq \tau = 0.8 
\end{align}
\end{definition}

In the above model, we see that Blue college accepts roughly $15\%$ of the applicants from both schools.  This implies that $\frac{P(Y=1|School=A)}{P(Y=1|School=B)}$ = 1, and so the model does not admit disparate impact and would be considered "fair" with respect to this fairness definition.  In fact, if we assume WLOG $P(Y=1|School=B) \le P(Y=1|School=A)$ then $\tau =1$ represents the \textit{fairest} possible outcome. Quite clearly, this model is not fair as it puts the bottom 85\% of students from School B at a disadvantage, while also offering an advantage to the top 15\% of students at school B.  

We simulate several years of admissions according to this fictitious model, but vary the acceptance rule as denoted in figure (?). A lower rule indicates that fewer students from both schools are accepted by admissions, where the $0$ rule in-dictates that no student from either case is accepted. 


We see that for any given year Blue College may be appear fair or unfair according to disparate impact, but also more importantly, we also see that the observed unfairness exhibited by the admissions data in aggregate reveals a fair trend despite obvious bias in the admissions.  Conversely, the Wasserstein distance reveals a fixed amount of bias for each rule, and also shows that the bias observed decreases as the rule trends towards zero.  Indeed, as the decision rule approaches the trivially fair scenario where all individuals from both school's are rejected, the Wasserstein distance decreases.  
\includegraphics[scale=.4]{graphics/di_stinks!.png}
